Efficient Computation of Positional Population Counts Using SIMD Instructions

In several fields such as statistics, machine learning, and bioinformatics, categorical variables are frequently represented as one-hot encoded vectors. For example, given 8 distinct values, we map each value to a byte where only a single bit has been set. We are motivated to quickly compute statistics over such encodings. Given a stream of k-bit words, we seek to compute k distinct sums corresponding to bit values at indexes 0, 1, 2, ..., k-1. If the k-bit words are one-hot encoded then the sums correspond to a frequency histogram. This multiple-sum problem is a generalization of the population-count problem where we seek the sum of all bit values. Accordingly, we refer to the multiple-sum problem as a positional population-count. Using SIMD (Single Instruction, Multiple Data) instructions from recent Intel processors, we describe algorithms for computing the 16-bit position population count using less than half of a CPU cycle per 16-bit word. Our best approach uses up to 400 times fewer instructions and is up to 50 times faster than baseline code using only regular (non-SIMD) instructions, for sufficiently large inputs.

==> extracontent.tex <==


\begin{table}
\caption{Host machines used for testing. Code was compiled using GCC 8 on all hosts.}
\label{table:systems-used}\centering
\begin{tabular}{lllll}
\toprule
\multirow{2}{*}{{Processor}} & \multirow{2}{*}{{Microarchitecture}} & \multicolumn{3}{c}{{Cache (KB)}} \\ \cline{3-5} 
                                    &                                             & {L1} & {L2} & {L3} \\ \midrule
Intel i3-8121U (10nm)      & Cannon Lake (x64)                   & 32+32     & 256     & 4096     \\
Intel Xeon E5-2697 v3 (22 nm) & Haswell (x64)                   & 32+32     & 256     & 35840    \\ \bottomrule
\end{tabular}
\end{table}


\daniel{I think we need a section where we explain how we go from a vectorized popcnt algo to a vectorized pospopcnt. The idea seems to work with bits, and then convert the bits into counters, somehow. }

\daniel{I suspect that this section should be called Harley-Seal Algorithm?}

\daniel{From this point forward, the paper is not likely to be understood. I would urge us very strongly to simplify.}

\daniel{It seems that the code has two different implementations of this idea, one that relies on AVX512VBMI, and I suspect it is what is benchmarked on Cannon Lake, and then one that relies on AVX512BW. Presumably, we only benchmark AVX512VBMI. Yet, oddly enough, there is no mention in the paper of AVX512VBMI at all, instead it refers to AVX512BW. }

\daniel{In any case, if we are going to refer to AVX512BW or AVX512VBMI (whichever it is), we should discuss it here (say what it is). If we are going to invoke something like AVX512BW, then people need to understand what it is and why they should care.}

Given the performance of the circuit-based Harley-Seal (HS)\cite{warren2007,mula2017faster} algorithm described for the canonical population count problem we investigated possible variations of this algorithm for the positional population count problem.
%The original HS-algorithm was inspired by carry-save adder (CSA) circuits (Fig.~\ref{fig:csa-network}) used to construct digital adders in microarchitectures and display extremely good performance metrics on larger inputs streams. 


%Without loss of generality, given three distinct 1-bit input values ($a,b,c \in \{0,1\}$) and 
%their 2-bit sum $a + b + c \in \{0,1,2,3\}$ it is possible to extract the least significant bit from the 2-bit sum using the bitwise expression
%$(a \oplus b) \oplus c$ and the most significant bit with $(a \land b) \lor ((a \oplus b) \land c)$. We can generalize this
%workflow to any standard integer such that three input words produce two output words, $h$ (high) and $l$ (low), corresponding to the 
%most and least significant bits, respectively (Fig.~\ref{fig:csa}). 

%\begin{figure}
%\centering
%\begin{cpp}[0.6\columnwidth]
%void CSA(uint64_t* h, uint64_t* l, 
%  uint64_t a, uint64_t b, uint64_t c)
%{
%  uint64_t u = a xor b;
%  *h = (a bitand b) bitor (u bitand c);
%  *l = u xor c;
%}
%\end{cpp}
%\caption{\label{fig:csa} Generalization of the %carry-save adder update step. Given three input values $a$, $b$, and $c$ we compute the
%most significant bit $h$ and least significant bit $l$. These output values are used in the next layer of the circuit.}
%\end{figure}

\daniel{This next bit is not clear. We write $1 \times \texttt{ones} + 2 \times \texttt{two} + 4 \times \texttt{fours} + \cdots$, presumably these are vectors of 5-bit values? Later we refer to things like \texttt{twosA} as being bits. I actually think that they are bits and that the notation $1 \times \texttt{ones} + 2 \times \texttt{two} + 4 \times \texttt{fours} + \cdots$ is a bit careless. }


In our implementation, CSA operators are combined into a 16-input circuit using five different 5-bit accumulators referred to as 
\texttt{ones}, \texttt{twos}, \texttt{fours}, \texttt{eights} and \texttt{sixteens} such that
the linear combination $1 \times \texttt{ones} + 2 \times \texttt{two} + 4 \times \texttt{fours} + 8 \times \texttt{eights} + 16 \times \texttt{sixteens}$ 
correspond to the final population count. All our implementations
operate on blocks of 16 vectors and proceeds as follows:

\begin{enumerate}
    \item Compute the high and low bits (CSA) from a zero-vector, and data words $d_0$ and $d_1$, and store
          the most significant bit (MSB\textsubscript{b}) in \texttt{twosA} and least significant bit (LSB\textsubscript{b}) to \texttt{ones}.
    \item Repeat step 1 for $d_2$ and $d_3$ and store the MSB\textsubscript{b} in \texttt{twosB}. At this point we have two bitvectors
          of MSB\textsubscript{b}s from four different input words $\{d_{0},d_{1},d_{2},d_{3}\}$.
    \item To proceed, we compute the high and low bits using the CSA subroutine with the arguments \texttt{twosA} and \texttt{twosB} 
          and store the MSB\textsubscript{b} in \texttt{foursA}.
    \item Start over and repeat step 1-3 with new input words $\{d_{4},d_{5},d_{6},d_{7}\}$. As in step 3, we now have
          a pair of bitvectors that we compute the high and low bits for \texttt{foursA} and \texttt{foursB} into \texttt{eightsA}.
    \item Repeat steps 1-4 with words $\{d_{8},d_{9},\ldots,d_{15}\}$ to get \texttt{eightsB}. Again, we can now compute 
          the high and low bits using \texttt{eightsA} and \texttt{eightsB} to get \texttt{sixteens}.
    \item The number of set bits in \texttt{sixteens} corresponds to 1/16 of the number of set bits in the
          last 16 input words. We compute the number of set bits using a population count and increment the partial sum accumulator.
    \item Repeat steps 1-6 until no more data is available. The residual counts in the partial 5-bit accumulators \texttt{ones}, \texttt{twos},
          \texttt{fours}, \texttt{eights} are multiplied with \{1, 2, 4, 8\} and added to the total count.
\end{enumerate}


\daniel{What is step 5? The step 5 in the enumeration above does not refer to the computation of a population count.}
Building on this idea of using circuits for counting bits, we derived a natural extension of the HS-based algorithm by 
replacing the population count of \texttt{sixteens} in step 5 with 16 separate
shift-add updates of partial sum accumulators corresponding to bit position $\{0,1,\ldots,15\}$. Care must be taken to ensure that the relatively small 16-bit 
accumulators do not overflow. To address this, we block the inner loop into steps of 65,535 iterations 
and update the output counters with the partial results following each blocked iteration.

\daniel{The next paragraph refers to two HS-based algorithms, but I am not sure what they are. And how to they relate to the AVX2 one.}

To analyze how the change from a population count to multiple partial accumulators affects performance 
between the two HS-based algorithms we focus on their AVX-512 implementations using the performance of the Cannon Lake architecture as reference. 
The \texttt{avx512\_popcount} function\cite{mula2017faster}  involves 10~instructions with a latency of 16~cycles
whereas the partial accumulator update step involves 3 instructions with a latency of 3 cycles~for a 
total of 48~instructions and 48~latency. We therefore expect the \texttt{pospopcnt} HS-algorithm to run slightly slower compared to its \texttt{popcnt} counterpart.

\daniel{We want to explain where the throughput and latency numbers come from. We refer to more than one implementation of AVX-512.}

\daniel{Daniel stopped here on October 9th 2019.}

\subsection{Tree-of-Adders and Forest-of-Adders}\label{sec:alg-forest}

Next we describe an algorithm based on trees-of-adders~\cite{KnuthV4A,Wilkes}
(Fig.~\ref{fig:tree-of-adders}) that performs well on moderately sized inputs. The
key insight to using a tree-of-adders for the conventional population count
problem is to recognize that the sum of two $n$-bit numbers is never wider than
$2n$ bits. By exploiting this property in an iterative fashion we can compute
the total sum in time proportional to the logarithm of the final sum bit-width.
For example, starting with 1-bit numbers, their sum require two bits of storage,
and pairs of 2-bit numbers require four bits of storage, and so on. This
property combined with large computer words (currently 64, 128, 256 or 512 bits
in commodity hardware) allows us to perform several such pairwise additions
simultaneously using bit-level parallelism. 

\begin{figure}
    \centering 
    \subfloat[\label{fig:tree-panel1}per-word population count]{\includegraphics[scale=1.1]{tree-adder-panel1.eps}}
    \subfloat[\label{fig:tree-panel2}positional population count]{\includegraphics[scale=1.1]{tree-adder-panel2}}\hspace{1cm}
    \caption{\label{fig:tree-of-adders} Overview of the difference between trees-of-adders used in population count and the proposed forest-of-adders for the positional population count.}
\end{figure}

It is possible to describe the same algorithmic approach for the positional
population count problem by maintaining $k$ separate trees-of-adders for bits
$[0, 1, \ldots, k)$ (Fig.~\ref{fig:tree-of-adders}). We call a collection of
trees-of-adders an \emph{adder forest}. So for a forest of 16 trees, we
conceptually process batches of 16 input values $b_0, b_1, \ldots, b_{15}$ as
follows:

\begin{enumerate}[noitemsep]
    \item Add the target bit $k$ of $b_0$ and $b_1$ shifted to most significant
        bit to get the 2-bit pairwise sum $s^2_{0,1}$.
    \item Repeat step 1 seven times with the words $\{2,3,\ldots,15\}$ to get
        $s^2_{2,3}$, $s^2_{4,5}$, $s^2_{6,7}$, $s^2_{8,9}$, $s^2_{10,11}$,
        $s^2_{12,13}$, and $s^2_{14,15}$.
    \item Sum together $s^2_{0,1}$ with $s^2_{2,3}$ to get $s^4_{0,3}$. Repeat
        three times to get $s^4_{4,7}$, $s^4_{8,11}$, and $s^4_{12,15}$.
    \item Sum together $s^4_{0,3}$ with $s^4_{4,7}$ to get $s^8_{0,7}$. Repeat
        this to get $s^8_{8,15}$.
    \item Sum together $s^8_{0,7}$ and $s^8_{8,15}$ to get the final count for
        the target bit.
    \item Repeat steps 1-5 for the remaining 15 bits in the forest.
\end{enumerate}

In practice we process trees in a memory-friendlier fashion by
updating all 16 trees for the current word pair before proceeding.


\subsection{Byte-blending}\label{sec:alg-blend}

When the input data is very small we cannot use the HS-based algorithm as it
operates on large blocks of 16 vectors. Addressing this, we describe an
efficient algorithm for small input data with much lower input limit. Without
loss of generality, given two 2-byte input words $d_0$ and $d_1$ we blend the
most-significant byte (MSB) of $d_0$ with the least-significant byte (LSB) of
$d_1$ and blend the LSB of $d_0$ with the MSB of $d_1$ into the words $b_0$ and
$b_1$. By using the \texttt{VPMOVB2M} (Packed MOVe Byte to Mask,
\texttt{\_mmNNN\_movemask\_epi8}, where \texttt{NNN} is empty, 256, or 512)
instruction, we extract the most-significant bit from each byte of $b_0$ and
$b_1$ into a target word and increment the target counter with its population count.
Next, we use the add instruction to shift $b_0$ and $b_1$ one bit to the left
($b_0 + b_0$ or $b_1 + b_1$) instead of using the actual shift instruction.
Although conceptually identical, the add operator has better throughput (0.33
clocks-per-instruction (CPI)) compared to an actual shift operation (1 CPI) on
most modern commodity processors. Finally, we compute the per-word population
count.

As an example implementation using 256-bit registers, given sixteen 32-bit words
$\{w_1, w_2, \ldots w_{16}\}$ from two registers we extract out the MSB from two
vectors into a new register of thirty-two 8-byte words. This is similarly done
for the LSB. Next, the most-significant bit for each byte is extracted using the
\texttt{VPMOVB2M} instruction resulting in a single 32-bit masked word. The
destination counters for bit 16 and 8 are updated with the population count of
the masked word for the MSB and LSB components, respectively. The next bit is
shifted in to the most-significant bit position using an add instruction. This
prodecure is repeated seven more times for bits $15 \rightarrow 9$ and $7
\rightarrow 1$.


\subsection{Microbenchmarking}

We performed microbenchmarks of the different subroutines to assess various performance metrics. First, we investigated 
the effect on performance with different input sizes (Fig.~\ref{fig:results-machines}). For very short input streams an unrolled SSE4-based implementation of the 
byte-blend algorithm (\texttt{sse\_blend\_popcnt\_unroll8}, see section \ref{sec:alg-scalar}) outperforms all AVX-512-based algorithms.\footnote{SSE4 instructions operate on 128-bit registers, unlike the 256-bit and 512-bit registers of AVX2 and AVX-512.}
This is unsurprising as the large register methods consume up to 512 values per iteration. At around 256 input values the AVX-512-methods display 
superior performance and continue to increase in throughput until around 65,536 input values. The Harley-Seal-based population count algorithm performs 
well up until exhausting low-level instruction and data cache (L1 cache, 32+32 KiB on our Cannon Lake machine) whereafter performance degrades slightly. We observe
another drop in performance when exhausting L2 cache (256 KiB). Remarkably, at this point the pospopcnt Harley-Seal-based algorithm have achieved 
parity in speed with the conventional Harley-Seal population count (Fig.~\ref{fig:results-machines}) with close to identical state paths (total number of cycles) despite executing 60\% more instructions. 
We performed the same experiments using Haswell-based architecture (Table~\ref{table:systems-used}) with similar results 
(Fig.~\ref{fig:results-machines} and Table~\ref{table:results-machines}).


%\begin{figure}
%\centering
%\includegraphics[width=\textwidth]{pposcnt-performance-range.eps}
%\caption{\label{fig:results-machines}Number of CPU cycles / 16-bit word as a function of %number of input values using the machines in Table ~\ref{table:systems-used}.}
%\end{figure}

\begin{figure}
    \centering 
    \subfloat[\label{fig:perf-cannonlake}per-word population count]{\includegraphics[clip,scale=1.5]{ppospopcnt-perf-cannonlake.pdf}}
    \subfloat[\label{fig:perf-haswell}positional population count]{\includegraphics[trim={0 0  0cm 0},clip,scale=1.5]{ppospopcnt-perf-haswell.pdf}}\hspace{1cm}
%\subfloat[positional population count as a popul]{\includegraphics[trim={0 0 0 0cm},clip,scale=1.5]{pospopcnt-overview-pane3}}
    \caption{\label{fig:results-machines}Number of CPU cycles / 16-bit word as a function of number of input values using the host machines listed in Table ~\ref{table:systems-used}.
    \hl{placeholder, rerunning} \hl{Be consistent, if we use Harley-Seal elsewhere, then write it as such in the figure, and so forth.}}
\end{figure}


\begin{table}
\centering
\caption{Performance metrics of the \texttt{pospopcnt} operation at 262,144 input values for Cannon Lake and Haswell host machines (Table~\ref{table:systems-used}). For reference, the \texttt{popcount} (AVX2 and AVX-512) functions compute the conventional population count.}
\label{table:results-machines}\centering
\begin{tabular}{lccc}
\hline
\multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{3}{c}{\textbf{Architecture: Cannon Lake}}                                                 \\ \cline{2-4} 
                                 & \textbf{Instructions / cycle} & \textbf{Cycles / 16-bit word} & \textbf{Instructions / 16-bit word} \\ \hline
popcount (AVX512BW)                  & 1.47                         & 0.12                          & 0.17                                \\
Byte-blend (AVX2, unrolled-8)    & 3.99                         & 0.75                          & 2.98                                \\
Byte-blend (AVX512BW, unrolled-8)    & 3.14                         & 0.55                          & 1.71                                \\
Adder-forest (AVX512BW)              & 2.25                         & 0.27                          & 0.61                                \\
Harley-Seal (AVX512BW)               & 2.19                         & 0.12                          & 0.26                                \\ 
Scalar (no SIMD)               & 3.82                         & 17.52                          & 67.00                                \\ \hline
\multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{3}{c}{\textbf{Architecture: Haswell}}                                                 \\ \cline{2-4} 
                                 & \textbf{Instructions / cycle} & \textbf{Cycles / 16-bit word} & \textbf{Instructions / 16-bit word} \\ \hline
popcount (AVX2)                  & 1.28                         & 0.27                          & 0.41                                \\
Byte-blend (SSE4, unrolled-8)    & 3.85                         & 1.49                          & 5.84                                \\
Byte-blend (AVX2, unrolled-8)    & 3.84                         & 0.75                          & 2.92                                \\
Adder-forest (AVX2)              & 2.94                         & 0.49                          & 1.46                                \\
Harley-Seal (AVX2)               & 1.92                         & 0.36                          & 0.69                                \\ 
Scalar (no SIMD)               & 3.82                         & 17.52                          & 67.00                                \\ \hline
\end{tabular}
\end{table}

To quantify the relative speedup, we compared the pospopcnt algorithms to the reference
method (Fig.~\ref{fig:pospopcnt-naive}) with auto-vectorization disabled resulting in scalar computation (Table~\ref{table:results-relative-nosimd}). Our proposed pospopcnt algorithms runs faster at all input sizes and achieves almost 140-fold improvement in speed compared to the non-SIMD version on larger inputs.

Taken together, we have demonstrated a significant acceleration of the novel pospopcnt-operation using SIMD instructions for different sizes of input streams. Furthermore, we have shown that the considerably more complex pospopcnt-operation can achieve parity in speed with the fastest known implementation of the canonical popcount-operation on large input streams\cite{mula2017faster} despite executing more instructions.

\begin{table}
\caption{Relative throughput compared to the scalar algorithm (Fig.~\ref{fig:pospopcnt-naive}) with vectorization explicitly disabled. For each count of input values, the best relative throughput is in bold.}
\label{table:results-relative-nosimd}\centering
\begin{tabular}{lllllllll}
    \toprule
    \multirow{2}{*}{{\textbf{Algorithm}}} & \multicolumn{8}{c}{{\textbf{Input values}}}                                                                                   \\ \cline{2-9} 
                                        & {\textbf{128}} & {\textbf{256}} & {\textbf{512}} & {\textbf{1024}} & {\textbf{2048}} & {\textbf{4096}} & {\textbf{8192}} & {\textbf{65536}} \\ \midrule
Byte-blend (SSE4, unrolled-8)    & \textbf{8.3} & 9.8      & 10.6     & 11.0        & 11.6     & 11.9     & 12.1     & 12.3      \\
Byte-blend (AVX512BW, unrolled-8) & 7.1     & \textbf{11.2} & \textbf{16.2} & 2        & 25.5     & 27.9     & 29.7     & 31.6      \\
Adder-forest (AVX512BW)         & 3.1     & 2.8      & 14.5     & \textbf{23.1} & \textbf{34.4} & 44.9     & 52.8     & 61.7      \\
Harley-Seal (AVX512BW)           & 2.1     & 2.3       & 8.2      & 15.1     & 28.2     & \textbf{49.1} & \textbf{76.1} & \textbf{138.7} \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Quality control of high-throughput sequencing data}

Over the last decade, large-scale international collaborative efforts have
amassed increasingly large and diverse sequencing datasets that are now
culminating in population-scaled national initiatives such as the UK 100,000
Genomes Project\cite{Turnbull2018}, and the US All of Us Research
Program\cite{AllofUs2019} that will encompass up to a million individuals with
sequenced genomes. In these projects, genomic sequencing with the use of
massively parallel high-throughput sequencing technologies generates hundreds of
millions of genomic fragments (reads) per sample. Sequencing reads that have
been mapped (aligned) to a reference sequence are frequently stored in the
incumbent SAM interchange format~\cite{Li2009}, its binary representation BAM, or in the column-oriented binary representation CRAM. Twelve distinct categories encoded as 1-hot encoded read states (Table
\ref{tab:sam-flag-description}) are stored as their union ($s_0 + s_1 + \ldots +s_{11}$ 
where $s_i$ is the encoding for category $i$) in a single machine word called the \texttt{FLAG} field. These
states encode information such as the orientation of the read and if the read
was successfully mapped to the reference. Computing summary statistics for this
field is frequently used as an important quality control step. The current
standard toolchain, SAMtools~\cite{Li2009}, implements this analysis using
heavily branched and scalar code. We investigated the potential application of
the positional popcount operation as a method for accelerating this scalar code.

\begin{longtable}{|l|l|l|l|}
\caption{\textbf{State description for the FLAG field.} Read states are
classified into 12 distinct categories ranging from its pairing information to
failing quality control checks such as being a likely PCR or optical duplicate.}
\label{tab:sam-flag-description}\\
\hline
\textbf{Bit} & \textbf{One-hot}                                     & \textbf{Description}                               & \textbf{Bit-field name}          \\ \hline
\endfirsthead
%
\endhead
%
1   & 00000000 0000000\textbf{1} & Read paired                               & \texttt{BAM\_FPAIRED}        \\ \hline
2   & 00000000 000000\textbf{1}0 & Read mapped in proper pair                & \texttt{BAM\_FPROPER\_PAIR}  \\ \hline
3   & 00000000 00000\textbf{1}00 & Read unmapped                             & \texttt{BAM\_FUNMAP}         \\ \hline
4   & 00000000 0000\textbf{1}000 & Mate unmapped                             & \texttt{BAM\_FMUNMAP}        \\ \hline
5   & 00000000 000\textbf{1}0000 & Read reverse strand                       & \texttt{BAM\_FREVERSE}       \\ \hline
6   & 00000000 00\textbf{1}00000 & Mate reverse strand                       & \texttt{BAM\_FMREVERSE}      \\ \hline
7   & 00000000 0\textbf{1}000000 & First in pair                             & \texttt{BAM\_FREAD1}         \\ \hline
8   & 00000000 \textbf{1}0000000 & Second in pair                            & \texttt{BAM\_FREAD2}         \\ \hline
9   & 0000000\textbf{1} 00000000 & Not primary alignment                     & \texttt{BAM\_FSECONDARY}     \\ \hline
10  & 000000\textbf{1}0 00000000 & Read fails platform/vendor quality checks & \texttt{BAM\_FQCFAIL}        \\ \hline
11  & 00000\textbf{1}00 00000000 & Read is PCR or optical duplicate          & \texttt{BAM\_FDUP}           \\ \hline
12  & 0000\textbf{1}000 00000000 & Supplementary alignment                   & \texttt{BAM\_FSUPPLEMENTARY} \\ \hline
\end{longtable}

The standard approach for computing summary statistics for the \texttt{FLAG}
field involves several bit-wise dependencies that introduce unavoidable branch
conditions (Figure \ref{fig:SAMtools-flagstats}). In addition, this statistic is
computed jointly for reads that pass quality control and those that do
not. Despite these limitation, the heavily branched and bit-dependent SAMtools
code can be rewritten using a mask-select propagate-carry approach that feeds
into Harley-Seal-based carry-save adder networks using SIMD instructions in four
steps (Figure \ref{fig:SAMtools-flagstats-simd}):

\begin{enumerate}[noitemsep]
    \item The bit-fields \texttt{BAM\_FUNMAP} and \texttt{BAM\_FDUP} are always counted.
    \item Rule 1: If the read has the bit-field \texttt{BAM\_FSECONDARY} set then mask all bits.
    \item Rule 2: If the read has the bit-field \texttt{BAM\_FSUPPLEMENTARY} set mask all bits.
    \item Count the remaining bit-fields (possible masked out by rule 1 or 2).
\end{enumerate}

{
\captionsetup{type=figure}
\begin{minted}{python}
for c in 1..n # Loop over FLAGs
  # Selector for passing QC or failing QC
  QC = 1 if (c & BAM_FQCFAIL) else 0
  if c & BAM_FSECONDARY: # Secondary read
    ++out[QC]["secondary"]
  elif c & BAM_FSUPPLEMENTARY: # Supplementary read
    ++out[QC]["supplementary"]
  elif c & BAM_FPAIRED: # Read is paired
    if (c & BAM_FPROPER_PAIR) && not (c & BAM_FUNMAP):
      ++out[QC]["n_pair_good"]
    if c & BAM_FREAD1: ++out[QC]["n_read1"]
    if c & BAM_FREAD2: ++out[QC]["n_read2"]
    if (c & BAM_FMUNMAP) && not (c & BAM_FUNMAP):
      ++out[QC]["n_sgltn"]
    if not (c & BAM_FUNMAP) && not (c & BAM_FMUNMAP):
      ++out[QC]["pair_map"]
  if not (c & BAM_FUNMAP): ++out[QC]["mapped"] # Is mapped
  if not (c & BAM_FDUP):   ++out[QC]["dup"] # Is not duplicated
\end{minted}
\captionof{figure}{\label{fig:SAMtools-flagstats}Pseudo-code for algorithm used
in SAMtools for computing summary statistics for \texttt{FLAG} values. Field names are
described in Table \ref{tab:sam-flag-description}. The original macro subroutine can
be found at
\url{https://github.com/SAMtools/SAMtools/blob/master/bam_stat.c\#L47}
(Last accessed: September 4, 2019)}
}

{
\captionsetup{type=figure}
\begin{minted}{python}
# Masks (rules)
mask1 = BAM_FSECONDARY + BAM_FSUPPLEMENTARY
mask2 = BAM_FUNMAP + BAM_FSECONDARY + BAM_FDUP + BAM_FSUPPLEMENTARY
mask3 = BAM_FQCFAIL

for c in 1..n # Loop over FLAGs
  # Mask operation: the assumption here is that predicate
  # evaluations result in either a one-mask (11...1) or a zero
  # mask (00...0) as they would for SIMD instructions prior to the 
  # AVX0512 ISA.
  dat = c & (((c & mask1) > 0) | mask2)
  # Branchless mask-select: if QC is not set then L is kept and LU
  # is zeroed out. Otherwise LU is kept and L is zeroed out.
  L  = dat & ((dat & mask3) == 0)
  LU = dat & ((dat & mask3) == mask3)
  out[0] = pospopcnt(L)  # count positional bits for not BAM_FQCFAIL
  out[1] = pospopcnt(LU) # count positional bits for BAM_FQCFAIL
\end{minted}
\captionof{figure}{\label{fig:SAMtools-flagstats-simd}Pseudo-code for SIMD-based
algorithm for a single update for a \texttt{FLAG} value.}
}

We benchmarked the difference between the positional popcount-based
algorithm and the reference implementation on a deeply sequenced human dataset
with >824 million reads\footnote{Downloaded from
\url{https://dnanexus-rnd.s3.amazonaws.com/NA12878-xten/mappings/NA12878D_HiSeqX_R1.bam}.
Last accessed: 29 July, 2019.}. In order to simulate a more realistic situation
where column projections are stored in contiguous blocks of memory (as in CRAM)
and require decompression prior to computation, we compressed \texttt{FLAG}
fields into contiguous blocks of 512 kb (8192 16-bit words) using the general
purpose compressors Lz4 (\url{https://lz4.github.io/lz4/}) or Zstd
(\url{https://facebook.github.io/zstd/}).

On this readset, the pospopcnt-based subroutine is up to 2562-fold faster
compared to the binary representation of SAM when using LZ4 and up to 3802-fold
faster when the input data is uncompressed (Table
\ref{tab:flagstats-pospopcnt}). The pospopcnt function was bounded by both disk
I/O and by decompression performance as around 80\% of CPU time is spent
retrieving and inflating data from disk. Arguably, this comparison is unfair as
the legacy SAM/BAM format have limited random access and no column projection
capabilities compared to the newer CRAM format~\cite{Hsi-YangFritz2011}. When
compared to CRAM, our proposed pospopcnt-based subroutine is still 402.6-fold
faster. Lastly, we investigated the potential speedup of the original scalar
subroutine in SAMtools by using efficient column projection and changing the
compression method to Lz4 for efficient decompression. This code refactoring
resulted in a massive 390.3-fold improvement in speed but remain 6.6-fold slower
compared to the pospopcnt-based subroutine (Table
\ref{tab:flagstats-pospopcnt-refactor}-\ref{tab:flagstats-pospopcnt-complete}).

\begin{longtable}{|l|l|l|}
\caption{\textbf{Completion time for SAMtools and pospopcnt.} The
pospopcnt-based algorithm is considerable faster compared to SAMtools using
either the standard binary interchange format BAM or the more modern
column-projection-capable format CRAM.}
\label{tab:flagstats-pospopcnt}\\
\hline
\textbf{Approach} & \textbf{Time} & \textbf{Speedup} \\ \hline
\endfirsthead
%
\endhead
%
SAMtools – BAM    & 30m 50.06s    & 1                \\ \hline
SAMtools – CRAM   & 4m 50.68s     & 6.36             \\ \hline
pospopcnt-LZ4         & 0.72s         & 2569.53          \\ \hline
pospopcnt-raw         & 0.48s         & 3802.90          \\ \hline
\end{longtable}

\begin{longtable}{|l|l|l|}
\caption{\textbf{Completion time for refactored SAMtools and pospopcnt.} After
refactoring SAMtools to support column-projection and using the general
compression engine LZ4, the pospopcnt-based approach is still considerably
faster.} 
\label{tab:flagstats-pospopcnt-refactor}\\
\hline
\textbf{Approach}    & \textbf{Time} & \textbf{Speedup} \\ \hline
\endfirsthead
%
\endhead
%
SAMtools-rewrite+LZ4 & 4.74 s        & 1                \\ \hline
pospopcnt            & 0.72s         & 6.58             \\ \hline
\end{longtable}

\begin{longtable}{|l|l|l|l|l|}
\caption{\textbf{Completion time for computing FLAG summary statistics}. \texttt{FLAG}
fields were compressed in blocks of 512 kB (8192 16-bit words) using the general
compression libraries LZ4 or Zstd. LZ4 can be used in two different modes: the
standard mode that compress faster but at worse fold compresion (LZ4) and in a
mode that compress better at slower speeds (LZ4-HC). All compression methods
were evaluated over their parameter space for compression: LZ4 (1-9) and Zstd
(1-20). Times are listed in milliseconds. Decompression times are included in
either algorithm for computing the \texttt{FLAG} summary statistic. The
SAM-branchless subroutine is described online at
\url{https://github.com/mklarqvist/FlagStats/}. Abbreviations: Comp. Method:
Compression Method; Decomp: Decompression.}
\label{tab:flagstats-pospopcnt-complete}\\
\hline
\textbf{Comp. Method} & \textbf{Decomp.} & \textbf{SAM-branchless} & \textbf{SAM} & \textbf{pospopcnt} \\ \hline
\endfirsthead
%
\endhead
%
LZ4-HC-c1             & 988              & 8924                    & 4991         & 1107               \\ \hline
LZ4-HC-c2             & 993              & 8848                    & 5076         & 1132               \\ \hline
LZ4-HC-c3             & 938              & 8686                    & 4930         & 1049               \\ \hline
LZ4-HC-c4             & 846              & 8803                    & 4876         & 933                \\ \hline
LZ4-HC-c5             & 824              & 8525                    & 5117         & 974                \\ \hline
LZ4-HC-c6             & 770              & 8536                    & 4774         & 851                \\ \hline
LZ4-HC-c7             & 680              & 8404                    & 4748         & 837                \\ \hline
LZ4-HC-c8             & 644              & 8453                    & \textbf{4662}         & 755                \\ \hline
LZ4-HC-c9             & \textbf{580}          & \textbf{8434}                    & 4740         & \textbf{722}            \\ \hline
LZ4-c2           & 814              & 8658                    & 4886         & 990                \\ \hline
LZ4-c3           & 837              & 8576                    & 4840         & 941                \\ \hline
LZ4-c4           & 889              & 8627                    & 4861         & 1026               \\ \hline
LZ4-c5           & 826              & 8590                    & 4885         & 1037               \\ \hline
LZ4-c6           & 823              & 8629                    & 5034         & 951                \\ \hline
LZ4-c7           & 837              & 8606                    & 4999         & 985                \\ \hline
LZ4-c8           & 834              & 8604                    & 4920         & 962                \\ \hline
LZ4-c9           & 853              & 8615                    & 4944         & 951                \\ \hline
Zstd-c1               & 3435             & 11438                   & 7798         & 3630               \\ \hline
Zstd-c2               & 3577             & 11231                   & 8110         & 3767               \\ \hline
Zstd-c3               & 3403             & 11250                   & 7922         & 3553               \\ \hline
Zstd-c4               & 3562             & 11223                   & 7949         & 3649               \\ \hline
Zstd-c5               & 2919             & 10584                   & 7263         & 2986               \\ \hline
Zstd-c6               & 2964             & 10680                   & 7545         & 3015               \\ \hline
Zstd-c7               & 2681             & 10591                   & 7067         & 2715               \\ \hline
Zstd-c8               & 2641             & 10523                   & 7103         & 2850               \\ \hline
Zstd-c9               & 2352             & 10453                   & 6669         & 2463               \\ \hline
Zstd-c10              & 2309             & 10094                   & 6756         & 2509               \\ \hline
Zstd-c11              & 2344             & 10018                   & 6430         & 2467               \\ \hline
Zstd-c12              & 2116             & 9916                    & 6242         & 2252               \\ \hline
Zstd-c13              & 2107             & 9844                    & 6183         & 2236               \\ \hline
Zstd-c14              & 1955             & 9616                    & 5969         & 2044               \\ \hline
Zstd-c15              & 1716             & 9562                    & 5807         & 1808               \\ \hline
Zstd-c16              & 1286             & 9208                    & 5592         & 1448               \\ \hline
Zstd-c17              & 1278             & 8996                    & 5592         & 1396               \\ \hline
Zstd-c18              & 1192             & 8907                    & 5294         & 1306               \\ \hline
Zstd-c19              & 1181             & 8931                    & 5362         & 1293               \\ \hline
Zstd-c20              & 1175             & 8982                    & 5369         & 1303               \\ \hline
\end{longtable}

This example application demonstrates the efficiency and inherent flexibility of
the pospopcnt-based algorithms. Using the pospopcnt operation as a replacement
for heavily branched code resulted in over >3,800-fold improvement in speed. We
expect these subroutines to enhance existing methods and tools for the
exploration of large genomics datasets in a variety of ways.

